Bandits Under The Influence (Extended Version)

Recommender systems should adapt to user interests as the latter evolve. A prevalent cause for the evolution of user interests is the influence of their social circle. In general, when the interests are not known, online algorithms that explore the recommendation space while also exploiting observed preferences are preferable. We present online recommendation algorithms rooted in the linear multi-armed bandit literature. Our bandit algorithms are tailored precisely to recommendation scenarios where user interests evolve under social influence. In particular, we show that our adaptations of the classic LinREL and Thompson Sampling algorithms maintain the same asymptotic regret bounds as in the non-social case. We validate our approach experimentally using both synthetic and real datasets.

==> old.tex <==
\section{Problem Formulation}

In what follows, we present our mathematical model, which consists of users in a social network receiving recommendation from a recommender system. The model assumes that user interests are dynamic, in that they are affected by the recommendations they receive, as well 
We use bold script ({e.g.}, $\x,\y,\ub,\vb$) to denote vectors, and capital script ({e.g.}, $A,B,H$) to denote matrices. For either matrices or vectors, we use $\geq$ to indicate element-wise inequalities. For symmetric matrices, we use $\succeq$ to indicate dominance in the positive semidefinite sense; in particular, $A\succeq 0$ implies that $A$ is positive semidefinite. For  square matrices $A$, we denote by $\trace(A),\diag(A)$, $\rank(A)$ the trace, diagonal and rank of $A$, respectively.
Finally, given an $n\times m$ matrix $A$, we denote by $\col:\reals^{n\times m}\to \reals^{nm}$ the column-major order representation of $A$: i.e., $\col(A)$ maps the elements of $A$ to a vector, by stacking the $m$ columns of $A$ on top of each other.


\subsection{Overview}\label{sec:overview}
Our model assumes that user interests are dynamic: they are affected both by recommendations users receive, as well as by how other users' interests evolve. In particular, our model of user behavior takes into account the following factors:
\begin{enumerate}
\item \emph{Inherent interests.} Our model accounts for an inherent predisposition users may have, e.g., towards particular topics or genres. This is static and does not change through time. %; it is captured by an ``inherent'' interest profile distribution attributed  to  each user. 
\item \emph{Attraction.} As per the mere-exposure effect, users %in our model 
may exhibit attractive behavior: if a type of content is shown very often by the recommendation service, this might reinforce the desire of a user to consume it. 
%In the case of attractive users, the recommendation service can increase a user's interest in a certain topic by showing more of this type of content.
\item \emph{Aversion.} Users may also exhibit aversive behavior: a user can grow tired of a topic that she sees very often, and may want to see something new or rare. % This desire for novelty or serendipity can lead to an attrition  effect: a user may desire once in a while to view topics that are recommended infrequently.
\item \emph{Social influence.} % The final factor affecting a user's interests  is social-influence: 
A user's behavior can be affected by what people in her social circle (e.g., her friends or family) are interested in. %as she may also desire items similar to those of 
 %are presently interested in.
\end{enumerate}
%We refer to the first three as the \emph{personal} components of a user's behavior, and the latter as the \emph{social} component of the user's behavior.

Under the joint effect of the factors above, suggestions made by the recommender  instigate an \emph{interest cascade} over the users. Suggestions alter user interests through attraction or aversion; in turn, these changes affect neighboring users as well, on account of their social behavior. These effects propagate dynamically over the users' social network.
Next, we formally describe how each of these factors is incorporated in our model.


\subsection{Recommender System and User Utilities} 
We consider $n$ users receiving recommendations from an  entity we call the recommender. We denote by $[n]\equiv\{1,2,\ldots,n\}$ the set of all users. At each time step $t\in \naturals$,
the recommender suggests an item to each user in $[n]$, selected from a catalog $C$ of available items. The user accrues a utility from the item recommended. As discussed below,  the recommender's goal is to suggest items that maximize the aggregate user utility, i.e., the social welfare.

Following the standard convention 
in recommender systems, we assume  factor-based  user utilities. At each $t\in \naturals$, each user $i\in[n]$ has an \emph{interest profile}
	represented by a $d$-dimensional vector $\ub_i(t) \in \reals^d$.
Moreover, the item recommended to user $i$ at time $t$ is represented by a  $d$-dimensional \emph{feature profile}
$\vb_i(t)\in \reals^d$. Then, the rating\footnote{In practice, \eqref{factor} best approximates \emph{centered} ratings, i.e., ratings offset by a global average across users.} a user $i$ would give to the item suggested to her at time $t$ is given by
\begin{align}r_i(t)=\langle\ub_i(t),\vb_i(t)\rangle +\varepsilon, \label{factor}\end{align}
where $\varepsilon$ is zero mean, finite variance noise (i.i.d.~across users and timeslots). Note that, as a result, the expected rating is given by 
\begin{align}\bar{r}_i(t)=\langle\ub_i(t),\vb_i(t)\rangle , \end{align}
the inner product between the interest and feature profiles  \cite{Koren:2008}\cite{Koren:2009}. 
 Intuitively, each coordinate of a feature profile can be perceived as an item-specific feature such as, e.g., a movie's genre or an article's topic. The corresponding coordinate in an interest profile captures the propensity of the user to react positively or negatively to this feature. 

A natural objective for the recommender is to maximize social welfare, i.e., recommend items that maximize $$\sum_{i\in [n]} r_i(t) = \mathbf{1}^\top \mathbf{r}(t),$$
where $\mathbf{r}(t)\in \reals^n$ is the vector of ratings. Put differently, each rating $r_i$, $i\in[n]$, can be thought of as a \emph{reward} that the recommender receives, and the objective then is to maximize the cumulative reward.
\begin{comment}
We call $F(\ub_i(t),\vb_i(t))$ the \emph{utility} of user $i$ from the suggested item at time $t$. 
Without loss of generality\footnote{Note that $F(\ub,\vb)=F({s}\ub,\frac{1}{s}\vb)$, for any scalar $s\in \reals$, so we can assume that either user or feature profiles have a bounded norm.}, we assume that the item profiles $\vb_i\in\reals^d$ are normalized, i.e.: $\|\vb_i(t)
\|_2=1$ for all $i\in [n]$, $t\in \naturals.$ 
Under this assumption, given that a user's profile is $\ub$, the best item to recommend to user $i$ is the one that yields the highest expected rating; indeed, this is $$\argmax_{\vb\in \reals^d: \|\vb\|_2=1} F(\ub,\vb)= {\ub}/{\|\ub\|_2}, $$
i.e., the item that maximizes the utility of a user $i$.  
Note that identifying items that maximize the \emph{aggregate} utility across users (i.e., the sum of expected ratings to suggested items), is a natural goal for the recommender.
\end{comment}
%Indeed, the item recommended to user $i$ at time $t$ that would yield the highes
%\note[Laks]{Very clear and tutorial in nature. Candidate to prune if space becomes an issue. KDD community shd be used to factor models.} 


\subsection{Interest Evolution}\label{sec:interestevol}
The evolution of user interests captures the four factors outlined in Section~\ref{sec:overview}. At each time step $t\in \naturals$, the interest profile of a user $i\in [n]$ is chosen alternately between either a \emph{personalized} or a \emph{social} behavior. If personalized, the behavior of a user is again selected among  three possible outcomes, each corresponding to inherent interests, attraction, and aversion, respectively. 

The selection of which of these four behaviors takes place at a given time step is random, and occurs independently of selections at other users as well as selections at previous time slots. We denote with $\beta\in[0,1]$ the probability that the user selects a social behavior at time slot $t$. The probability of selecting a personalized behavior is thus $1\!-\!\beta$. Interests at these two distinct events are
as follows:

\medskip\noindent\textbf{Personalized Behavior.}  If a user's interest is selected through a personalized behavior, the user selects her profile through one of the three personalized factors outlined in Section~\ref{sec:overview}. In particular, for every $i\in [n]$, there exist probabilities $ \alpha_i,\gamma_i,\delta_i\in [0,1]$ such that $\alpha_i+\gamma_i+\delta_i=1$, and:
 \begin{itemize}
\item\textbf{Inherent interests.} With probability $\alpha_i$, user $i$ follows her \emph{inherent
	interests}.  That is, $\ub_i(t)$ is sampled from a probability distribution $\mu_i^0$ over $\reals^d$.
	This distribution does not vary with $t$ and captures the user's inherent predisposition. %For ease of exposition, we assume all $\mu_i^0$ have bounded support.
\item\textbf{Attraction.} With probability $\gamma_i$, user $i$ selects a profile that is \emph{attracted} to the items suggested to her in the past. To capture this notion denote by  $\mathcal{V}_i(t) = \{\vb_i(\tau)\}_{\tau\leq t}$ the \emph{history} of (profiles of) items suggested to a user $i$. Then, the interest of a user under attraction is given by $g(\mathcal{V}_i(t-1))$, a weighted average of the items suggested to it in the past. That is:
\begin{align}\ub_i(t) = g(\mathcal{V}_i(t-1)) = \frac{\sum_{\tau =0}^{t-1}  w_{t-\tau}\vb(\tau)}{\sum_{\tau =0}^{t-1}w_{t-\tau}}. \label{attraction}\end{align}
\item\textbf{Aversion.} With probability $\delta_i$, user $i$ selects a profile that is \emph{repulsed} by the items suggested to her in the past; that is, her interest profile is given by
\begin{align}\ub_i(t) = -g(\mathcal{V}_i(t-1)) = -\frac{\sum_{\tau =0}^{t-1}  w_{t-\tau}\vb(\tau)}{\sum_{\tau =0}^{t-1}w_{t-\tau}}. \label{aversion}\end{align}
\end{itemize}

To gain some intuition on \eqref{attraction} and \eqref{aversion}, recall that a user's utility at time $t$ is given by \eqref{factor}. Therefore, a profile generated under \eqref{attraction} implies that the suggestion that \emph{maximizes} her utility at time $t$ would be one that aligns perfectly (i.e., points in the same direction as) the weighted average $g$ up to time $t-1$. In contrast, under the aversive behavior \eqref{aversion}, the same suggestion \emph{minimizes} the user's utility.

Note that the weighted average $g$ is fully determined by the sequence weights $\{w_\tau\}_{\tau\in\naturals}$. By selecting decaying weights, a higher importance can be placed on more recent suggestions.

\smallskip\noindent\textbf{Social Behavior.} User $i$'s profile is selected through social behavior with probability $\beta$. Conditioned on this event:
\begin{itemize}
\item\textbf{Social Influence.} A user aligns her interests with a user $j$ selected from her social circle with probability $P_{ij}$. That is:
\begin{align}\ub_i(t) = \ub_{j}(t-1),\quad \text{with probability }P_{ij},\label{social} \end{align}
where $\sum_{j}P_{ij}=1$.
\end{itemize} The probability $P_{ij}\in[0,1]$ captures the influence that user $j$ has on user $i$. Note that users $j$ for which $P_{ij}=0$ (i.e., outside $i$'s social circle) have no influence on $i$. Moreover,  the set of pairs $(i,j)$ s.t. $P_{ij}\ne 0$, defines the social network among users.  We denote by $P\in [0,1]^{n\times n}$  the stochastic matrix with elements $P_{ij}$, $i,j\in [n]$; we assume that $P$ is ergodic (i.e., irreducible and aperiodic) \cite{gallager1996discrete}.

%\note[Laks]{Why should the i/c influence probs on a user sum to 1? What does it mean?} 

\medskip
%Under these dynamics, interests evolve in the form of a dynamic cascade: suggestions made by the recommender act as a forcing function, altering interests either through attraction or aversion. Such changes propagate across users through the social network. 
%\note[Laks]{It'd be nice if we could demonstrate this empirically.} 

\begin{comment}
\subsection{Recommended Item Distribution} \label{sec:recstrategy} %\label{sec:recobjective}

In practice, the recommender has access to a finite ``catalog'' of items. Recalling that feature profiles have norm 1, the recommender's catalog can be represented as a set $C\subseteq \mathbb{B}$, where $\mathbb{B}=\{\vb\in \reals^d:\|\vb\|_2 = 1\}$ is the set of items of norm 1 (i.e., the $d$-dimensional unit ball).  

We assume that the recommender selects the items $\vb_j(t)\in \mathbb{B}$ suggested to user $i\in [n]$ by sampling them from a discrete distribution $\nu_i$ over $\mathbb{B}$, whose support is $C$. Note that the expected feature profile of a suggested item is a weighted average among the vectors in $C$. As such, it belongs to the \emph{convex hull} of catalog $C$; formally:
\begin{align}
\bar{\vb}_i &= \int_{\vb\in \mathbb{B}}\vb d\nu_i \in \conv(C) \label{barv},
\end{align}
 Note that $\conv(C)$ is a convex polytope included in $\mathbb{B}$. 

The steady state user utilities depend only on the expectations $\bar{\vb}_i$, $i\in [n]$, rather than the entire distributions $\nu_i$.  We will thus refer to $\{\bar{\vb}_i\}_{i\in [n]}$ as the \emph{recommender strategy}; it is worth keeping in mind that, given a $\bar{\vb}_i\in \conv(C)$, finding a $\nu_i$ such that \eqref{barv} holds can be computed in polynomial time in $|C|$.

We further assume that the catalog $C$ is large; in particular,
for large catalog size $|C|$, we have:\begin{align}\conv(C)\simeq \mathbb{B}. \label{approx}\end{align}
This would be true if, for example, each item in the catalog are generated in an  i.i.d.~fashion from a distribution that covers the entire ball $\mathbb{B}$; this distribution need not  be uniform\footnote{Formally, $\lim_{|C|\to\infty}\conv(C) = \mathbb{B}$ w.p.~1 if, e.g., items in catalog $C$ are sampled independently from a probability distribution absolutely continuous to the uniform distribution on $\mathbb{B}$.}.
We revisit the issue of how to pick a distribution $\nu_i$ given $\bar{\vb}_i$, as well as how to interpret our results in the case of a finite catalog, in Section~\ref{sec:finite}.
%Assume that, at each time $t$, the recommender suggests an item with profile $\vb_j(t)$ sampled in an from a distribution $\nu_i$ over the unit ball $\{\vb\in \reals^d:\|\vb\|_2 = 1\}$, independently of the selection at other users as well as the selection at previous time steps. In practise, the support of this distribution cannot be the entire unit ball: in reality, the distribution $\nu$ must be discrete, and profiles selected with non-zero probability will be limited to profiles of items in the recommender's ``catalog''. However, if the catalog of the recommender is large, assuming that this distribution is continuous over $\mathbb{B}$ is a reasonable approximation. 

%\note[Laks]{I wonder if this assumption is really necessary. IIUC, we want to say the RS should maximize the average social welfare (in the limit as the horizon becomes infinite). The only difference between making this assumption and not is whether the RS gets to recommend one of the items in its catalog or an imaginary item. We ceratinly want the former so I don't understand why we need this assumption.} 

\subsection{Recommendation Objective}\label{sec:recobjective}

Observe that, under the above dynamics, the evolution of the system is a Markov chain, whose state comprises the interest and feature profiles. We define the objective of the recommender as maximizing the social welfare, i.e., the sum of expected user utilities, in \emph{steady state}. Formally, we wish to determine a strategy $\{\bar{\vb}_i\}_{i\in [n]}$ (and, hence, distributions $\nu_i$)  that maximizes:
\begin{align}\lim_{T\to\infty}\frac{1}{T}\sum_{t=0}^T\sum_{i\in[n]} \langle\ub_i(t),\vb_i(t)\rangle = \lim_{t\to\infty}\sum_{i\in[n]} \Exp[\langle\ub_i(t),\vb_i(t)\rangle],\label{reward}\end{align}
where the equality above holds w.p.~1 by the renewal theorem~\cite{gallager1996discrete}. %, as the process $\{\ub_i(t),\vb_i(t)\}_{i\in [n],i\in \naturals}$ is an ergodic Markov chain.
It is important to note that, under the interest dynamics described in \ref{sec:interestevol}, optimal recommendations to a user $i$ cannot be obtained independently of recommendations to other users: %User  $i$'s interests are affected by those of her neighbors, which, in turn may be affected through aversion or attraction towards the suggestions made by the recommender. Hence,
user $i$'s profile depends  on recommendations made not only directly to this use  on recommendations made not only directly to this user, but also  to any user reachable through $i$'s social network.

\end{comment}


\subsection{Online Setting}

In an online setting, we do not a priori assume knowledge of model parameters, particularly inherent profiles and attraction/aversion probabilities $\gamma,\delta$. We would nevertheless wish to propose an online algorithm maximizing  \eqref{factor}, e.g., over a finite horizon, etc.

To study this setting, we will assume that when presented with a recommendation $\vb$, the reward of a user $i$ follows \eqref{factor} \emph{in expectation}. Put differently, the reward is given by \eqref{factor} plus zero-mean noise.

We can consider the following partial online settings.

\noindent\textbf{No Social Network}. In this case, w.l.o.g. we can focus on a single user. In this case, the user's interest evolve as:
\begin{align}\ub(t)= \alpha \ub_0 + \gamma g(\mathcal{V}(t-1)) +\delta h(\mathcal{V}(t-1)),\label{nosocial}\end{align}
where $g,h$ may not necessarily be the same as above. In particular, it makes sense to start with something simple, where
$g(\mathcal{V}(t-1)) = \vb(t)$ and $g(\mathcal{V}(t-1)) = -\vb(t)$.

Note that if $\gamma=\delta=0$, maximizing \eqref{factor} while learning amounts to a linear bandit problem. What we would like to figure out is if, e.g., regret bounds can be provided if we incorporate attraction and aversion thusly. 

More generally, it would be good to study ``sticky'' arms in which rewards depend on previous actions, particularly through \eqref{factor} or more generally depending on some function of $\mathcal{V}(t-1)$. This setting is similar to non-stochastic (or adversarial) bandits~\cite{auer2002nonstochastic}\cite{ryabko2008learning}\cite{odalric2011adaptive}.

\noindent\textbf{Social Network Alone.} In the social network case, the matrix of profiles $U\in \reals^{n\times d}$ would evolve as
\begin{align}U(t) = \alpha U^0 + \beta P U(t-1),\label{snalone}\end{align}
for an appropriately defined weight matrix $P\in [0,1]^{n\times n}$. The goal here would be to again exploit while learning $P$, $U^0$. 

We should certainly assume we know the support of $P$. However, it makes sense to think of this also assuming we fully know $P$ and are trying to explore/exploit $U^0$.

\subsection{Social Network Alone}

The social network alone setting \eqref{snalone} can be seen as a deviation from the standard linear bandit setting. In particular, applying \eqref{snalone} recursively we get:
\begin{align}
U(t) &= \alpha U^0 + \beta\alpha P U^0 + \beta ^2 \alpha P^2 U^0 +\ldots (\beta P)^t \alpha U^0\\
& = A(t) U^0
%\\ & = \sum_{k=0}^t \right(\beta P \left)^k\alpha U^0
\end{align}
for $t\geq 1$, where \begin{align}
A(t) = \alpha \sum_{k=0}^t \left(\beta P \right)^k \in \mathbb{R}^{n\times n}.
\end{align}
Suppose now that at any time $t$ the recommender can choose recommendations from some finite subset $\mathcal{B}_t\subset\mathbb{B}$.  
Then, the ``arms'' are the possible recommendations $V(t)\in \mathbb{R}^{n\times d}$, which is a matrix whose rows are selected from $\mathcal{B}_t$ (note that there are $|\mathcal{B}_t|^n $ matrices to choose from).

Then the total expected reward is given by:
\begin{align}
\bar{r}_t &= \langle A(t) U^0, V(t)\rangle = \trace(A(t)U^0 V^{\top}(t))\nonumber\\
& =\trace( U^0 V^\top (t) A(t))
=\langle U^0, A(t)^\top V(t)\rangle.  \label{rew}
\end{align}
where $\langle A, B\rangle = \mathop{\trace}(AB^\top).$

\noindent\textbf{Remark 1.} If we assume that $\alpha,\beta,P$ are known, then so is $A(t)$. Then, the setting is exactly a linear bandits setting, where the environment $\mathcal{B}_t$ is multiplied by $A(t)$, and the unknown parameter is $U^0$  Studying this may still be non-trivial, due to the exponential nature of arms; maybe that is easy to tackle though, because of the specific nature/structure of the problem. If not an alternative is to use something like \cite{jun2017scalable} which purports dealing with scalability. In general, knowing that the reward has form \eqref{rew} might lead to a faster/better algorithm than using, e.g., \cite{li2017provably,chu2011contextual} directly/na\"ively. This may indeed arise if, e.g., $\mathcal{B}_t=\mathcal{B}$, i.e., the choices of recommendations are fixed. In this case, the "context" changes in a predictable way, and computation up to time $t$ might be useful to speed up/save computation at time $t+1$.

\noindent\textbf{Remark 2.} Things probably get more interesting if we assume, e.g., that both $P$ \emph{and} $U^0$ are unknown. Assuming that $U^0$ is known and $P$ is unknown is also an interesting step, as the latter is linear in $A(t)$ but not on $P$. In particular, this is an interesting "network inference" problem.

\subsection{No Social Network Setting}

Something to look here is if things become easy/reduce to standard setting if the environment becomes a $2d$-dimensional vector $[\vb(t);\vb(t-1)]$, and/or using \cite{odalric2011adaptive,auer2002nonstochastic}.


\section{Online Algorithms for Social Bandits}

We cast the regret minimization problem into a linear/contextual bandit setting. For consistency with existing algorithms like \linrel and \linucb, we first vectorize the representation of recommendations and rewards.

To that end, we define $$\mathbf{u}_0\equiv \mathtt{vec}(U^0)\in \reals^{nd}$$  as the $nd$-dimensional vector resulting from representing $U^0$ row-wise. Assuming $P,\alpha,\beta$ are known, we can set $\mathbf{u}_0$ is the underlying unknown parameter yielding the rewards.


Recall that $\mathbf{v}_i(t)\in \mathcal{B}\subseteq \reals^{d}$ be the recommendation to user $i$, and $V(t)$ is the corresponding $n\times d$ matrix. We will assume that $\mathbf{v}_i(t)$, $i\in D$ can be selected from a set $\mathcal{B}\subseteq \reals^d$, where we consider the following cases
\begin{itemize}
\item $\mathcal{B}=\mathbb{B}$, i.e., recommendations can be selected from the unit ball.
\item $\mathcal{B}$ is a convex subset of $\reals^d$.
\item $\mathcal{B}\subset\reals^d$ is a finite subset, i.e., a ``catalog'' of possible recommendations.
\end{itemize}
Given a $V\in \reals^{n\times d}$, we define its row-wise vector representation as:
$$\mathbf{v} = \vect(V) = [\mathbf{v}_1^\top,\mathbf{v}_2^\top, \ldots,\mathbf{v_n}]^\top\in \mathbb{B}^n \subseteq \reals^{nd}. $$
%Let also $mathbf{a}_i\in \reals^d$ $i=1,\ldots,n$ be the $i$-th row of $A(t)^\top$. 
We also define the ``arms'' at time $t$ as a matrix $X(V(t),A(t))\in \reals^{n\times nd}$ s.t.:

\begin{align}X(V,A) \equiv \left[ \begin{matrix}
a_{11} \mathbf{v}_1^\top &  a_{12} \mathbf{v}_1^\top & \ldots &  a_{1n} \mathbf{v}_1^\top\\
a_{21} \mathbf{v}_2^\top &  a_{22} \mathbf{v}_2^\top & \ldots &  a_{2n} \mathbf{v}_2^\top\\
& \vdots& \ddots & \vdots\\
a_{n1} \mathbf{v}_n^\top &  a_{n2} \mathbf{v}_n^\top & \ldots &  a_{nn} \mathbf{v}_n^\top\\
  \end{matrix}
\right]\label{xarms}
\end{align}
 Then, the  expected rewards at all users are given by vector $\mathbf{r}(t)\in \reals^n$, where:
\begin{align}
\bar{\mathbf{r}}(t) &= \diag( A(t) U^0 V^\top(t) ) = X(V(t),A(t)) \mathbf{u}_0
\end{align}
Note also that, in vector form, the total reward (sum across all rewards) is:
\begin{align}\bar{r}(t) = \mathbf{u}_0^
\top \vect(A^\top(t) V) =\mathbf{u}_0^\top   L(t) \mathbf{v}\in \reals
 \end{align}
where
 the matrix 
 \begin{align}
	 L(t)\equiv  A(t)^\top \otimes I_d\in \reals^{nd\times nd}
 \end{align}
 is the $nd\times nd$ matrix resulting from the Kronecker product of $A(t)^\top$ with the identity matrix $I_d\in \reals^{d\times d}$.
%$V$ ranges among the $\mathcal{B}_t^n$ options we have for each of the matrices $V\in\mathcal{B}_t^n$.
%\begin{align}\mathbf{v}=[v_1;v_2;\ldots;v_n]=\mathtt{vec}(V)\in (\mathcal{B}_t)^n.
%\end{align}
%Let $\mathbf{A}(t)\in \reals^{nd\times nd}$ be a block diagonal matrix with $A(t)$ replicated in its diagonal. Then, $$"x_{a,t}"=\mathbf{A}(t)\mathbf{v}(t).$$
The total expected reward at time $t$ under recommendations $V$ is then given by:
%\begin{align}
%r(t) = \mathbf{u}_0^\top \mathbf{A}(t) \mathbf{v}(t) 
%\end{align}
\begin{align}
	\bar{r}(t) =  \mathbf{u}_0^\top L(t) \mathbf{v} = \trace(U^0, A^\top (t) V(t)) = \mathbf{1}^\top X(V(t),A(t))) \mathbf{u}_0 
\end{align}

\subsection{\linrel}

The \linrel algorithm \cite{auer2003confidence}, also called ``confidence ball'' in \cite{dani2008stochastic}, operates under the following assumptions:
\begin{itemize}
\item Arms are sampled from a set $\mathcal{A}\subseteq \reals^d$, possibly uncountable.
\item The expected loss is given by:
	\begin{align}\bar{\ell}(t)=\expect[\ell(t)\mid \mathcal{H}_t] = \mathbf{x}_t^\top \mathbf{\theta}\label{theirs} \end{align}
where  $\mathcal{H}_t$ is the history up to time $t$ and $\mathbf{\theta} \in \reals^d$. 
\end{itemize}
 The algorithm proceeds as follows:
\begin{itemize}
\item $d$ arms that span $\mathcal{A}$ are played first.
\item At iteration $t\geq d$, arm $\mathbf{x}_t\in \mathcal{A}$ is played, where
	\begin{align}\label{min} \mathbf{x}_t = \mathop{\arg\min}_{\mathbf{x}\in \mathcal{A}} \min_{\mathbf{z}\in 
		\mathcal{C}^2_t} \mathbf{z}^\top \mathbf{x}\end{align}
		where $\mathcal{C}^2_t$ is defined as follows. First, as usual,
		$\hat{\mathbf{\theta}}_t$ is constructed via linear regression from past observations as:
		$$\hat{\mathbf{\theta}}_t  = (X_{t-1}^\top X_{t-1})^{-1}X^\top_{t-1} {\boldsymbol \ell} _{t-1}$$
and  
		$$\mathcal{C}^2_t = \left\{\mathbf{z}: \|\mathbf{z}-\hat{\mathbf{\theta}}_t\|_{2,Z_t}\leq \sqrt{\beta_t}\right\}$$
		for $\beta=\beta(t,d,\delta)$ some closed form function of $t$, $d$, and a parameter $\delta$, $Z_t=X_{t-1}^\top X_{t-1}$, and $$\|\mathbf{x}\|_{2,A} = \sqrt{\mathbf{x}^\top A\mathbf{x}}.$$
An alternative algorithm optimizes over $C_t^1$, which is similarly defined as:
		$$\mathcal{C}^1_t = \left\{\mathbf{z}: \|\mathbf{z}-\hat{\mathbf{\theta}}_t\|_{1,Z_t}\leq \sqrt{n\beta_t}\right\},$$
and
$$\|\mathbf{x}\|_{1,A} = \|A^{1/2}\mathbf{x}\|_1 $$

\end{itemize}


To cast our scenario into this setting, we define our loss to be the negative reward. That is
\begin{align*}{\boldsymbol \ell}(t) &= -\textbf{r}(t),\quad  \text{and the aggregate reward is } \ell(t)= -\mathbf{1}^\top\textbf{r}_t \end{align*}
Note that the loss is indeed of the form \eqref{theirs}, using $\theta=-\ub_0$ as a parameter vector.
In our case:
\begin{itemize}
\item At each iteration, we pull $n$ arms, one for each user.
\item There are $nd$ parameters to learn, so the ``warmup'' phase must involve $d$ recommendations/simultaneous pulls of these $n$ arms.
	\item Vectors $\mathbf{x}_t$ relate to recommendations $V$ as before; that is, ``arms'' interacting with each individual user are given by $X(V(t),A(t))$, as defined in \eqref{xarms}.
\item We can compute again $\hat{\mathbf{u}}_0$ through the appropriate regression over $X(V,A)$ and the rewards $\mathbf{r}_t$, as follows:
$$\hat{\mathbf{u}}_0 (t) = \argmin_{\mathbf{u}\in \reals^{nd}}\sum_{\tau=1}^{t-1} \|X(V(\tau),A(\tau))\mathbf{u} - \mathbf{r}_\tau\|_2^2.$$
\item The matrix $Z(t)\in \reals^{nd\times nd}$ is given by:
\begin{align*}
 Z(t) &= \sum_{\tau=1}^{t-1} \sum_{i=1}^n \mathbf{x}_i(\tau)  \mathbf{x}_i(\tau)^\top\\
 &=\sum_{\tau=1}^{t-1}X(V_\tau,A_\tau)^\top X(V_\tau,A_\tau),
\end{align*}

where
$$ \mathbf{x}_i = \left[ \begin{matrix}
a_{i1} \mathbf{v}_i^\top &  a_{12} \mathbf{v}_i^\top & \ldots &  a_{in} \mathbf{v}_i^\top 
\end{matrix}\right]
$$
is the $i$-th row of matrix $X$.
\item The optimization at each step becomes:
\begin{subequations} \label{eq:main}
\begin{align}
\text{Maximize:} &\quad \mathbf{u}^\top L(t)\mathbf{v} \label{ourobj}\\
\text{subject to:} & \quad\mathbf{v}\in \mathcal{B}^{(n)}\\
&\quad \|\hat{\mathbf{u}}_0-\mathbf{u}\|_{2,Z(t)}\leq \sqrt{\beta_t} \label{u0constr}
\end{align}
\end{subequations}
Note that $\hat{\ub}_0$ appears \emph{with a positive sign} in \eqref{u0constr}, precisely because, in our setting, $\theta\equiv-\ub_0$. Moreover, for the same reason, the minimization objective \eqref{min} should be
$$\text{Minimize:}\quad -\mathbf{u}^\top L(t)v  $$
which is the same as \eqref{ourobj}.
\end{itemize}
We therefore discuss how to solve  optimization problem \eqref{eq:main} for different values of set $\mathcal{B}$. We drop the dependence on $t$ for simplicity.


\begin{itemize}
\item \textbf{Euclidian ball, $\mathcal{C}^2$ constraints.} Consider the case that:
$$ \mathcal{B} = \mathbb{B}=\{\vb\in \reals^d:\|\vb\|_2 = 1\}.$$
Then, for a given $\mathbf{z}\in \reals^{nd}$, we have 
\begin{align}
\max_{\mathbf{v}\in \mathbb{B}^{(n)} } \mathbf{z}^\top \mathbf{v} = \sum_{i=1}^n \|\mathbf{z}_i\|_2 
\end{align}
where $\mathbf{z}_i\in \reals^d$ is the $i$-th sub-vector of dimension $d$ in $\mathbf{z}=[\mathbf{z}_1,\ldots,\mathbf{z}_n]$. To see this, note that the objective and constraints are separable over $\mathbf{v}_i\in \reals^d$, $i=1,\ldots,n$, and the optimal solution for each $i$ is attained at $\mathbf{v}_i = \mathbf{z}_i/\|\mathbf{z}_i\|_2$. Hence, \eqref{eq:main} becomes:
\begin{align}
\text{Maximize:} &\quad \sum_{i=1}^n \|\mathbf{z}_i\|_2\\
\text{subject to:} & \quad \mathbf{z}_i = (\mathbf{u}^\top L)_i, i=1,\ldots,n\\
& \|\hat{\mathbf{u}}_0-\mathbf{u}\|_{2,Z(t)}\leq \sqrt{\beta_t}
.\end{align}
This is \emph{not} a convex optimization problem. Nevertheless, it is a quadratic optimization problem with a single quadratic constraint, so it can be solved in polynomial time: see \cite{boyd2004convex}, Appendix B.
\item \textbf{$\mathcal{C}^1$ constraints.} In the case where we use $\ell_1$ norm constraints, several sets can be solved. All of them rely/exploit the fact that the optimization problem:

\begin{align*}
\text{Maximize:} &\quad \mathbf{u}^\top \mathbf{z}\\
\text{subject to:} &  
\quad \|\hat{\mathbf{u}}_0-\mathbf{u}\|_{1,Z}\leq c
\end{align*}
attains its maximum at one of the $2nd$ extreme points of the polytope $ \|\mathbf{u}+\hat{\mathbf{u}}_0\|_{2,Z}\leq c
$.
Hence, for $\mathcal{E}$ the set of these extreme points, we can solve  $|\mathcal{E}|=nd$ optimization problems of the form:
\begin{subequations}
\begin{align}
\text{Maximize:} &\quad \mathbf{u}^\top  L\mathbf{v} \\
\text{subject to:} & \quad\mathbf{v}\in \mathcal{B}^{(n)},
\end{align}
\label{eq:l1red}
\end{subequations}
\noindent with $\mathbf{u}$ being one of the $2nd$ vectors in $\mathcal{E}$.
 Note that in all cases the optimization \eqref{eq:l1red} is separable over $\mathbf{v}_i$, and thus itself reduces to solving $n$ problems. In conclusion, \eqref{eq:main} reduces to solving $n^2d$ problems of the form:
\begin{subequations}
\begin{align}
\text{Maximize:} &\quad \mathbf{z}^\top \mathbf{v}_i   \\
\text{subject to:} & \quad\mathbf{v}_i\in \mathcal{B},
\end{align}
\label{eq:l1red2}
\end{subequations}
\noindent for appropriately defined $\mathbf{z}\in \reals^d$.
We can therefore deal with $\mathcal{B}$ being (a) an arbitrary convex set (euclidian ball, convex polytope), \emph{as well as} (b) a finite subset of $\reals^d$!
\end{itemize}



\subsection{\linucb}

Going with the variant of \linucb suggested in \cite{li2017provably} (its generalized variant), a learner needs to select at time $t$ an arm $a\in \mathcal{A}(t)$. Each arm is associated with a context
$$x_{a,t} \in \reals^d.$$ There is an unknown $\theta\in \reals^d$ such that the reward observed by pulling an arm with $x_{a,t}=x$ is given by
$$r(t) = x^\top \theta + \varepsilon_t$$
where $\{\varepsilon_t\}_{t\in \naturals}$ are i.i.d., zero mean, finite variance, etc.

The algorithm proceeds as follows: 
\begin{itemize}
\item For $a_t \in \mathcal{A}(t)$ the arm selected at time $t$, the learner keeps track of the history $$X_t=[x_{a_\tau,\tau}]_{\tau=1}^t\in \reals^{t\times d}$$
of arms selected, as well as the rewards vector $y_t=[r(\tau)]_{\tau=1}^t\in \reals^t$
\item At time $t+1$, the learner estimates $\theta$ by solving the least squares problem:
$$\hat{\theta}_{t+1} = \argmin_{\theta} \|X_t \theta - y_t\|_2^2$$
\item The next arm is selected via algorithm:
$$a_{t+1} = \argmax_{a\in \mathcal{A}(t+1)}  \left(  x_{a,t+1} \hat{\theta}_{t+1} + c \cdot x_{a,t+1}^\top \Sigma_{t+1} x_{a,t+1} \right)$$
where $\Sigma_{t+1} = (X_t^\top X_t)^{-1}$ is the covariance of the estimate $\hat{\theta}_{t+1}$.


\noindent\textbf{Reminder of Notation.}
Then, the  expected rewards at all users are given by vector $\mathbf{r}(t)\in \reals^n$, where:
\begin{align}
\bar{\mathbf{r}}(t) &= \diag( A(t) U^0 V^\top(t) ) = X(V(t),A(t)) \mathbf{u}_0
\end{align}
Note also that, in vector form, the total reward (sum across all rewards) is:
\begin{align}\bar{r}(t) = \mathbf{u}_0^
\top \vect(A^\top(t) V) =\mathbf{u}_0^\top   L(t) \mathbf{v}\in \reals
 \end{align}
where
 the matrix 
 \begin{align}
	 L(t)\equiv  A(t)^\top \otimes I_d\in \reals^{nd\times nd}
 \end{align}
 is the $nd\times nd$ matrix resulting from the Kronecker product of $A(t)^\top$ with the identity matrix $I_d\in \reals^{d\times d}$.

\noindent\textbf{Social Network Alone}. Let's apply this to our setting. The unknown parameters are $\mathbf{u}_0$, and their estimation would be via linear regression as in \textsc{LinRel}: 
$$\hat{\mathbf{u}}_0 (t) = \argmin_{\mathbf{u}\in \reals^{nd}}\sum_{\tau=1}^{t-1} \|X(V(\tau),A(\tau))\mathbf{u} - \mathbf{r}_\tau\|_2^2.$$

The covariance of this estimate is 
$\Sigma_t = Z(t)^{-1}$, where again
the matrix $Z(t)\in \reals^{nd\times nd}$ is given by:
\begin{align*}
 Z(t) &= \sum_{\tau=1}^{t-1} \sum_{i=1}^n \mathbf{x}_i(\tau)  \mathbf{x}_i(\tau)^\top\\
 &=\sum_{\tau=1}^{t-1}X(V_\tau,A_\tau)^\top X(V_\tau,A_\tau),
\end{align*}
where
$$ \mathbf{x}_i = \left[ \begin{matrix}
a_{i1} \mathbf{v}_i^\top &  a_{12} \mathbf{v}_i^\top & \ldots &  a_{in} \mathbf{v}_i^\top 
\end{matrix}\right]\in \mathbb{R}^{nd}
$$
Then \linucb would select
\begin{align}
\argmax_{V\in (\mathcal{B})^n} \left(\hat{\mathbf{u}}_{t}^\top L(t) \mathbf{v}  + c \cdot \mathbf{v}^\top L(t)^\top \Sigma_{t} L(t) \mathbf{v}  \right) \label{eq:select}\end{align}

\begin{comment}

In our setting, let's treat $$\mathbf{u}_0=\mathtt{vec}(U^0)\in \reals^{nd}$$  as the row-wise vector resulting from $U^0$. Assuming $P,\alpha,\beta$ are known, we can set $\theta=\mathbf{u}_0$.

Let $v_i(t)\in \mathcal{B}_t\subseteq \reals^{d}$ be the recommendation to user $i$. %Let also $mathbf{a}_i\in \reals^d$ $i=1,\ldots,n$ be the $i$-th row of $A(t)^\top$. 
Then the arms that we have available at time $t$ are:
\begin{align}x_{V,t} = \mathtt{vec}(A(t)^\top V) \end{align}
where $V$ ranges among the $|\mathcal{B}_t|^n$ options we have for each of the matrices $V\in\mathcal{B}_t^n$.
%\begin{align}\mathbf{v}=[v_1;v_2;\ldots;v_n]=\mathtt{vec}(V)\in (\mathcal{B}_t)^n.
%\end{align}
%Let $\mathbf{A}(t)\in \reals^{nd\times nd}$ be a block diagonal matrix with $A(t)$ replicated in its diagonal. Then, $$"x_{a,t}"=\mathbf{A}(t)\mathbf{v}(t).$$
The expected reward at time $t$ is
%\begin{align}
%r(t) = \mathbf{u}_0^\top \mathbf{A}(t) \mathbf{v}(t) 
%\end{align}
\begin{align}
r(t) = \mathbf{u}_0^\top x_{V(t),t} = \trace(U^0, A^\top (t) V(t))
\end{align}

Then \linucb would select
\begin{align}
\argmax_{V\in (\mathcal{B}_t)^n} \left(\hat{\mathbf{u}}_{t+1}^\top x_{V,t} + c \cdot x_{V,t}^\top \Sigma_{t+1} x_{V,t}  \right) \label{eq:select}\end{align}
where 
$$\Sigma_{t+1} = \left(\sum_{\tau=1}^t x_{V(\tau),\tau}x_{V(\tau),\tau}^\top\right)^{-1}  $$

We can write:
\begin{align}
x_{V,t} = \mathtt{vec}(A(t)^\top V) \stackrel{}{=} \mathbf{A}(t) \mathbf{v}\in \reals^{nd}
\end{align}
for some $\mathbf{A}(t)\in \reals^{nd\times nd}$, where vector $\mathbf{}v$ is
\begin{align}\mathbf{v}=[v_1;v_2;\ldots;v_n]=\mathtt{vec}(V)\in (\mathcal{B}_t)^n,
\end{align}
and the matrix $\mathbf{A}(t)$ contains $n$ blocks of $d$ rows, where in block $i$, the "diagonal" is formed of the row $i$, $a^T_i(t)$, and $0$ in the other cells:
$$\begin{bmatrix}
    a_{11} & a_{12} & \dots & a_{1n} & 0 & \dots \\
    0 & 0 & \dots & 0 & a_{11} & a_{12} & \dots & a_{1n} & \dots\\
    \dots
\end{bmatrix} $$

Then the optimization problem becomes:
\begin{align}
\argmax_{
\mathbf{v}\in (\mathcal{B}_t)^n} \left(\hat{\mathbf{u}}_{t+1}^\top \mathbf{A}(t)\mathbf{v} + c \cdot \mathbf{v}^\top \mathbf{A}(t)^\top \Sigma_{t+1} \mathbf{A}(t)\mathbf{v} \right), \label{eq:select_new}\end{align}
where 
$$\Sigma_{t+1} = \left(\sum_{\tau=1}^t x_{V(\tau),\tau}x_{V(\tau),\tau}^\top\right)^{-1}  = \left(\sum_{\tau=1}^t \mathbf{A}(\tau) \mathbf{v}(\tau)\mathbf{v}^\top(\tau)\mathbf{A}^\top(\tau)\right)^{-1}  $$
Given that we can write $x_{V,t}$ this way, the optimization \eqref{eq:select} becomes a non-convex optimization problem with a quadratic objective. if $$\mathcal{B}_t=\mathbb{B}=\{v\in\reals^d: \|v\|\leq 1\}$$ then an approximate solution can be constructed via SDP relaxation.
\end{comment}

 This is a non-convex problem. In the case where:
 $$\mathcal{B}_t=\mathbb{B}=\{v\in\reals^d: \|v\|\leq 1\}$$
 approximate solution can be constructed via SDP relaxation.


\paragraph*{TODO}:
\begin{enumerate}
\item how can we compute $x_{V,t}$ incrementally?
\item can we find an polynomial algorithm using SDP relaxation?
\item other algorithms, if we cannot find bounds for \linucb?
\item applied to our setting, can we avoid an exponential number of arms?
\end{enumerate}




\subsection{\linucb revisited (our setting)}
\linucb operates under the following assumptions:
\begin{itemize}
\item Arms $ \mathbf{v}_t$ are sampled from a set $\mathcal{A}\subseteq \reals^{nd}$, possibly uncountable.
\item The expected reward is given by:
	\begin{align} \expect[r_t\mid \mathcal{H}_t] = \mathbf{u_0}^\top L(t) \mathbf{v}_t = \mathbf{u_0}^\top \mathbf{x}_t  \label{linucbOrig} \in \reals\end{align}
where  $\mathcal{H}_t$ is the history up to time $t$,  $\mathbf{u_o} = \mathtt{vec}(U^0) \in \reals^{nd}$, and $ \mathbf{x}_t$ is defined as 
\begin{align}  \mathbf{x}_t = L(t)  \mathbf{v}_t \label{xt}\end{align} for $ \mathbf{v}_t \in \reals^{nd}$ being the recommended items. 

\item We can compute again $\hat{\mathbf{u}}_0$ by  the least-squares estimator, as follows:
$$\hat{\mathbf{u}}_0 (t) = \argmin_{\mathbf{u_0}\in \reals^{nd}}\sum_{\tau=1}^{t-1} (\mathbf{u_0}^\top \mathbf{x}_t - \mathbf{r}_\tau)^2$$
\item The matrix $Z_t\in \reals^{nd\times nd}$ is given by:
$$ Z_t = \sum_{\tau=1}^{t-1}  \mathbf{x}_\tau  \mathbf{x}_\tau^\top, $$
\item the solution for $\hat{\mathbf{u}}_0 (t)$ can be obtained by 
\begin{align} \hat{\mathbf{u}}_0 (t) = Z_t^{-1} \sum_{\tau=1}^{t-1} x_t r_t \label{u0hat}\end{align}

\item the confidence set around  $\hat{\mathbf{u}}_0 (t)$ can be set by 
$$\mathcal{C}_t = \left\{\mathbf{u} \in \reals^{nd}: \|\mathbf{u}-\hat{\mathbf{u}}_0(t)\|_{2,Z_{t} }\leq \beta_t\right\},$$

\item the optimization at each step becomes: 
\begin{subequations} \label{eq:main}
\begin{align}
\text{Maximize:} &\quad \mathbf{u}^\top L(t)\mathbf{v} \label{ourobj}\\
\text{subject to:} & \quad\mathbf{v}\in \mathcal{B}^{(n)}\\
&\quad \|\mathbf{u} - \hat{\mathbf{u}}_0\|_{2,Z_{t}}\leq \beta_t \label{u0constr}
\end{align}
\end{subequations}

\end{itemize}

==> results.tex <==
\section{Results}

We present here the full results for the experimental section. Figure~\ref{fig:results_fs_full} and Figure~\ref{fig:results_l2_full} show the results for the finite set and $L_2$ case respectively. Figure~\ref{fig:results_beta_full} shows the results for the $\beta_t$ parameter for both finite and $L_2$ cases. Tables~\ref{tab:comp_types_l2},\ref{tab:comp_sigma_l2}, and~\ref{tab:comp_nets_l2} show the varying parameter results for the $L_2$ case.
\begin{figure*}[!t]
    \subfloat[$N=10$, $d=5$, $m=100$]{\includegraphics[width=0.45\textwidth]{figures/reward_cmp_n10_d5_M100_sigma1_scale0.00001.pdf}}
    ~
    \subfloat[$N=10$, $d=5$, $m=1000$]{\includegraphics[width=0.45\textwidth]{figures/reward_cmp_n10_d5_M1000_sigma1_scale0.00001.pdf}}
    
    \subfloat[$N=100$, $d=20$, $m=100$]{\includegraphics[width=0.45\textwidth]{figures/reward_cmp_n100_d5_M1000_sigma1_scale0.000001.pdf}}
    ~
    \subfloat[$N=100$, $d=20$, $m=1000$]{\includegraphics[width=0.45\textwidth]{figures/reward_cmp_n100_d20_M1000_sigma1_scale0.000001.pdf}}
    
    \caption{Finite set; setup: horizon $100$, $\sigma=1$, $10^{-5}$ 
    $\beta$ scale}\label{fig:results_fs_full}
\end{figure*}

\begin{figure*}[!t]
  \subfloat[$n=10$, $d=5$]{\includegraphics[width=0.45\textwidth]{figures/reward_cmp_n10_d5_l2ball_sigma1_scale0.00001.pdf}}
  ~
  \subfloat[$n=10$, $d=10$]{\includegraphics[width=0.45\textwidth]{figures/reward_cmp_n10_d10_l2ball_sigma1_scale0.00001.pdf}}
  
  \subfloat[$n=100$, $d=5$]{\includegraphics[width=0.45\textwidth]{figures/reward_cmp_n100_d5_l2ball_sigma1_scale0.000001.pdf}}
  ~
  \subfloat[$n=100$, $d=20$]{\includegraphics[width=0.45\textwidth]{figures/reward_cmp_n100_d20_l2ball_sigma1_scale0.000001.pdf}}
  
  \caption{$L_2$ ball case; setup: horizon $100$, 
  $\sigma=1$, $10^{-5}$ $\beta$ scale}\label{fig:results_l2_full}
\end{figure*}

\begin{figure*}
    \subfloat[$\beta$ scale, finite set]{\includegraphics[width=0.45\textwidth]{figures/reward_scale_cmp_n10_d5_M100_sigma1.pdf}}
    ~
    \subfloat[$\beta$ scale, $L_2$ ball]{\includegraphics[width=0.45\textwidth]{figures/reward_scale_cmp_n10_d5_l2ball_sigma1.pdf}}
    
    \caption{Regret at horizon $100$ obtained for various values of the $\beta$ scale; lower values are better.}\label{fig:results_beta_full}
\end{figure*}

\begin{table}\centering
  \caption{Regret at horizon $100$ obtained for various $\sigma$ values, $L_2$ ball case; lower values are better.}\label{tab:comp_sigma_l2}
  \begin{tabular}{crrr}
    \toprule
    Method&$\sigma=2$&$\sigma=1$&$\sigma=0.1$\\
    \midrule
    \textsc{LinREL1}& $314.07$ & $218.24$ & $107.82$\\
    \textsc{ThompsonSampling}& $159.50$ & $157.71$ & $136.23$\\
    \textsc{Regression}& $379.71$ & $379.71$ & $379.71$\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}\centering
  \caption{Regret at horizon $100$ obtained for various methods of computing $A$ (expectation default, stochastic, fix-point $A_\infty$), $L_2$ ball; lower values are better.}\label{tab:comp_types_l2}
  \begin{tabular}{crrr}
    \toprule
    Method& &stoch.&$A_\infty$\\
    \midrule
    \textsc{LinREL1}& $217.24$ & $238.15$ & $242.80$\\
    \textsc{ThompsonSampling}& $157.71$ & $285.57$ & $446.83$\\
    \textsc{Regression}& $379.71$ & $457.00$ & $446.83$\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}\centering
  \caption{Regret at horizon $100$ obtained for various synthetic graph models, $L_2$ ball case, $n=100$.}\label{tab:comp_nets_l2}
  \begin{tabular}{crrr}
    \toprule
    Method& cmp.& ER & BA\\
    \midrule
    \textsc{LinREL1}& $1538.59$ & $1616.38$ & $1584.60$\\
    \textsc{ThompsonSampling}& $1147.94$ & $2086.91$ & $1215.80$\\
    \textsc{Regression}& $2007.14$ & $2086.91$ & $1937.72$ \\
    \bottomrule
  \end{tabular}
\end{table}
